GFG -- Gender-Fair Generation: A CALAMITA Challenge

Gender-fair language aims at promoting gender equality by using terms and expressions that include all identities and avoid reinforcing gender stereotypes. Implementing gender-fair strategies is particularly challenging in heavily gender-marked languages, such as Italian. To address this, the Gender-Fair Generation challenge intends to help shift toward gender-fair language in written communication. The challenge, designed to assess and monitor the recognition and generation of gender-fair language in both mono- and cross-lingual scenarios, includes three tasks: (1) the detection of gendered expressions in Italian sentences, (2) the reformulation of gendered expressions into gender-fair alternatives, and (3) the generation of gender-fair language in automatic translation from English to Italian. The challenge relies on three different annotated datasets: the GFL-it corpus, which contains Italian texts extracted from administrative documents provided by the University of Brescia; GeNTE, a bilingual test set for gender-neutral rewriting and translation built upon a subset of the Europarl dataset; and Neo-GATE, a bilingual test set designed to assess the use of non-binary neomorphemes in Italian for both fair formulation and translation tasks. Finally, each task is evaluated with specific metrics: average of F1-score obtained by means of BERTScore computed on each entry of the datasets for task 1, an accuracy measured with a gender-neutral classifier, and a coverage-weighted accuracy for tasks 2 and 3.

==> Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto

==> backup.tex <==
GeNTE is a parallel English-Italian test set \citep{piergentili-etal-2023-gender}. 
Originally designed to evaluate MT models' ability to perform gender-neutral translations, 
GeNTE was built as a subset of the Europarl corpus \citep{koehn2005europarl}, which  
is representative of natural, formal communicative situations from the institutional domain, the context where gender-neutral language is most accepted and encouraged \cite{piergentili-etal-2023-gender, piergentili-etal-2023-hi}. 
Overall, it consists of 1500  <\textit{English source, Gendered Italian reference, Neutral Italian reference}> triplets aligned at the sentence level, which always contain at least one mention to human referents.
The gendered Italian reference (REF-G) come from the original Europarl corpus, whereas the neutral reference (REF-N)  was produced by professional translators that edited gendered forms into neutral alternatives.

As shown in Table \ref{tab:gente_examples}, GeNTE  represents two types of phenomena, which are equally represented within the corpus. Namely, \textit{i)} \texttt{Set-N}, featuring 750 
gender-ambiguous source 
sentences that require to be rendered in a neutral manner; and 
\textsc{Set-G}
featuring gender-unambiguous source sentences, to
be properly rendered with gendered (masculine or feminine) forms. 
Crucially these two sets are a key feature of GeNTE, as they allows to benchmark whether systems are able to perform gender-neutral translations, but only when desirable. As a matter of fact,  when referents' gender is unknown or irrelevant, undue gender inferences should not
be made and neutral language should be used. However, neutralization should not be always enforced, and when a referent's gender is relevant and known, models should not over-generalize to neutral generations.

Accordingly, we propose the use of the whole GeNTE test set for the cross-lingual task 3, testing models' ability to produce neutral translations only when appropriate. For task 2, we only repurpose the Italian portion of the corpus, including \textsc{Set-N} sentences, only. 
